The Traffic Reaction Model: A kinetic compartmental approach to road traffic modeling

In this work, a family of finite volume discretization schemes for LWR-type first order traffic flow models (with possible on- and off-ramps) is proposed: the Traffic Reaction Model (TRM). These schemes yield systems of ODEs that are formally equivalent to the kinetic systems used to model chemical reaction networks. An in-depth numerical analysis of the TRM is performed. On the one hand, the analytical properties of the scheme (nonnegative, conservative, capacity-preserving, monotone) and its relation to more traditional schemes for traffic flow models (Godunov, CTM) are presented. Finally, the link between the TRM and kinetic systems is exploited to offer a novel compartmental interpretation of traffic models. In particular, kinetic theory is used to derive dynamical properties (namely persistence and Lyapunov stability) of the TRM for a specific road configuration. Two extensions of the proposed model, to networks and changing driving conditions, are also described.

==> reaction_rates.tex <==

\begin{tikzpicture}[x=\textwidth,y=0.2\textwidth]


\draw[-{Latex[length=3mm,width=2mm]}] (0,1) -- (1,1) node[anchor=west]{$x$};
\draw (0.2,1.05) node[anchor=south]{$x_{j-1}$} -- (0.2,0.95) ;
\draw (0.5,1.05) node[anchor=south] (tot) {$x_{j}$} -- (0.5,0.95) ;
\draw (0.8,1.05) node[anchor=south]{$x_{j+1}$} -- (0.8,0.95) ;


\draw[thick] (0.01,0.75) -- (0.99,0.75);
\draw[thick](0.01,0.45) -- (0.99,0.45);


\draw[thick] (0.01,0.2) -- (0.99,0.2);
\draw[thick](0.01,-0.1) -- (0.99,-0.1);


\draw[dashed,red] (0.05,1)  -- (0.05,-0.3);
\draw[dashed,red] (0.35,1)    -- (0.35,-0.3) node[anchor=north] {{\large $\displaystyle S_{j}+N_{j-1}\mathop{\rightarrow} N_j + S_{j-1}$}};
\draw[dashed,red] (0.65,1)  -- (0.65,-0.3) node[anchor=north] {{\large $S_{j+1}+N_{j}\mathop{\rightarrow} N_{j+1} + S_{j}$}};
\draw[dashed,red] (0.95,1)  -- (0.95,-0.3);

\draw (0.2,0.325) node {$j-1$};
\draw (0.5,0.325) node {$j$};
\draw (0.8,0.325) node {$j+1$};

\draw (0.825,0.6) node {\includegraphics[scale=0.7]{fig/car.png}};
\draw (0.1,0.6) node {\includegraphics[scale=0.7]{fig/car.png}};
\draw (0.2,0.6) node {\includegraphics[scale=0.7]{fig/car.png}};
\draw (0.4,0.6) node {\includegraphics[scale=0.7]{fig/car.png}};
\draw (0.5,0.6) node {\includegraphics[scale=0.7]{fig/car.png}};
\draw (0.575,0.6) node {\includegraphics[scale=0.7]{fig/car.png}};

\draw (0.5,0) node {$N_j$};
\draw (0.45,0.08) node {$N_j$};
\draw (0.57,0.08) node {$S_j$};
\draw (0.41,-0.04) node {$S_j$};
\draw (0.61,-0.03) node {$N_j$};
\draw (0.38,0.12) node {$N_j$};
\draw (0.53,0.12) node {$N_j$};


\draw (0.08,0) node {$S_{j-1}$};
\draw (0.15,0.0) node {$S_{j-1}$};
\draw (0.2,0.07) node {$N_{j-1}$};
\draw (0.3,-0.04) node {$S_{j-1}$};
\draw (0.25,-0.03) node {$S_{j-1}$};
\draw (0.1,0.12) node {$N_{j-1}$};
\draw (0.32,0.12) node {$N_{j-1}$};

\draw (0.9,0.05) node {$S_{j+1}$};
\draw (0.77,0.1) node {$S_{j+1}$};
\draw (0.85,-0.02) node {$N_{j+1}$};
\draw (0.72,-0.04) node {$S_{j+1}$};
\draw (0.68,0.1) node {$N_{j+1}$};
\draw (0.82,0.12) node {$N_{j+1}$};


%\draw[latex-latex] (0.35,0.0) -- (0.65,0.0) node[midway, below] {$\Delta x$};



\end{tikzpicture}


==> sk_cell.tex <==
\begin{tikzpicture}[x=\textwidth,y=0.15\textwidth]


\draw[thick,dashed,red] (0.2,0.25) -- (0.25,0.25) node[above] {$w_l$};
\draw[thick,red] (0.25,0.25) -- (0.5,0.25);
\draw[thick,red](0.5,0.85) -- (0.75,0.85);
\draw[thick,dashed,red](0.75,0.85) node[above] {$w_r$} -- (0.8,0.85) ;
\draw[thick,red](0.5,0.85) -- (0.5,0.25);


\draw[thick,blue, dotted] (0.25,0.25) -- (0.6,0.25);
\draw[thick,blue, dotted](0.6,0.85) -- (0.75,0.85);
\draw[thick,blue, dotted](0.6,0.85) -- (0.6,0.25);
\draw[-latex,blue] (0.5,0.55) -- (0.6,0.55) node[midway, below] {$\alpha \Delta t >0$};

\draw[thick,blue, dotted] (0.25,0.25) -- (0.4,0.25);
\draw[thick,blue, dotted](0.4,0.85) -- (0.75,0.85);
\draw[thick,blue, dotted](0.4,0.85) -- (0.4,0.25);
\draw[-latex,blue] (0.5,0.45) -- (0.4,0.45) node[midway, below] {$\alpha \Delta t <0$};

\draw[dashed] (0.35,1) -- (0.35,-0.1);
\draw[dashed] (0.5,1) -- (0.5,-0.1);
\draw[dashed] (0.65,1) -- (0.65,-0.1);



\draw[-{Latex[length=3mm,width=2mm]}] (0.2,0.15) -- (0.8,0.15) node[anchor=west]{$x$};
\draw (0.35,0.12) node[anchor=north east]{$-\Delta x/2$} -- (0.35,0.18) ;
\draw (0.5,0.12) node[anchor=north east] (tot) {$0$} -- (0.5,0.18) ;
\draw (0.65,0.12) node[anchor=north east]{$\Delta x/2$} -- (0.65,0.18) ;



\draw[decorate,decoration={brace,mirror}] (0.35,0) -- (0.5,0) node[below,midway,yshift=-5pt] { $I^-(\alpha,w_l,w_r)$};

\draw[decorate,decoration={brace,mirror}] (0.5,-0) -- (0.65,-0) node[below,midway,yshift=-5pt] { $I^+(\alpha,w_l,w_r)$};

\end{tikzpicture}


==> sk_half.tex <==



\begin{tikzpicture}[x=\textwidth,y=0.15\textwidth]


\draw[thick] (0.01,0.75) -- (0.99,0.75);
\draw[thick](0.01,0.45) -- (0.99,0.45);


\draw[dashed] (0.05,1) -- (0.05,0.1);
\draw[dashed] (0.35,1) -- (0.35,0.1);
\draw[dashed] (0.65,1) -- (0.65,0.1);
\draw[dashed] (0.95,1) -- (0.95,0.1);

\draw[] (0.05,0.75) -- (0.05,0.45);
\draw[dashed] (0.35,0.75) -- (0.35,0.45);
\draw[dashed] (0.65,0.75) -- (0.65,0.45);
\draw[dashed] (0.95,0.75) -- (0.95,0.45);

\draw (0.2,0.9) node {$(i-1)$-th cell};
\draw (0.5,0.9) node {$i$-th cell};
\draw (0.8,0.9) node {$(i+1)$-th cell};

\draw[-{Latex[length=3mm,width=2mm]}] (0,0.15) -- (1,0.15) node[anchor=west]{$x$};
\draw (0.2,0.12) node[anchor=north]{$x_{i-1}$} -- (0.2,0.18) ;
\draw (0.5,0.12) node[anchor=north] (tot) {$x_{i}$} -- (0.5,0.18) ;
\draw (0.8,0.12) node[anchor=north]{$x_{i+1}$} -- (0.8,0.18) ;

\draw (0.35,0.12) node[anchor=north]{$x_{i}-\Delta x/2$} -- (0.35,0.18) ;
\draw (0.65,0.12) node[anchor=north]{$x_{i}+\Delta x/2$} -- (0.65,0.18) ;


\draw (0.425,0.6) node {Left half};
\draw (0.575,0.6) node {Right half};


\draw[dashed,red] (0.5,0.15) -- (0.5,0.75);
\draw[dashed,red] (0.8,0.15) -- (0.8,0.75);
\draw[dashed,red] (0.2,0.15) -- (0.2,0.75);


%\draw[decorate,decoration={brace,mirror}] (0.35,0) -- (0.5,0) node[below,midway,yshift=-5pt] { $J_l(t_n,x_i)$};

%\draw[decorate,decoration={brace,mirror}] (0.5,-0) -- (0.65,-0) node[below,midway,yshift=-5pt] { $J_r(t_n,x_i)$};


\end{tikzpicture}




